Mnemosyne: Learning to Train Transformers with Transformers

In this work, we propose a new class of learnable optimizers, called \textit{Mnemosyne}. It is based on the novel spatio-temporal low-rank implicit attention Transformers that can learn to train entire neural network architectures, including other Transformers, without any task-specific optimizer tuning. We show that Mnemosyne: (a) outperforms popular LSTM optimizers (also with new feature engineering to mitigate catastrophic forgetting of LSTMs), (b) can successfully train Transformers while using simple meta-training strategies that require minimal computational resources, (c) matches accuracy-wise SOTA hand-designed optimizers with carefully tuned hyper-parameters (often producing top performing models). Furthermore, Mnemosyne provides space complexity comparable to that of its hand-designed first-order counterparts, which allows it to scale to training larger sets of parameters. We conduct an extensive empirical evaluation of Mnemosyne on: (a) fine-tuning a wide range of Vision Transformers (ViTs) from medium-size architectures to massive ViT-Hs (36 layers, 16 heads), (b) pre-training BERT models and (c) soft prompt-tuning large 11B+ T5XXL models. We complement our results with a comprehensive theoretical analysis of the compact associative memory used by Mnemosyne which we believe was never done before.

==> causal.tex <==
\subsection{Causal Mnemosyne for ML Training}
\label{sec:causal}

\begin{figure*}\vspace{-2mm}
  \begin{center}
  % \includegraphics[width=0.6\textwidth]{img/legend.pdf} \\
  \includegraphics[trim={0 0 1.8cm 0},clip,width=0.33\textwidth]{img/mnist_vit_long_horizon.pdf}
  \includegraphics[trim={0 0 1.8cm 0},clip,width=0.33\textwidth]{img/cifar10_vit.pdf}
  \includegraphics[trim={0 0 1.8cm 0},clip,width=0.33\textwidth]{img/cifar100_vit.pdf}
  \end{center}
\vspace{-6mm}
\caption{\small{Validation loss curves while training Vision Transfomer with Mnemosyne compared to other methods for image classification on $3$ different datasets, \textbf{left:} MNIST, \textbf{center:} CIFAR10 and \textbf{right:} CIFAR100 are shown.}}
\label{fig:vit}
\vspace{-4mm}
\end{figure*}

\textbf{Preliminaries:}
In this setting, Mnemosyne's optimizer $g^{\mathrm{hist}}_{\theta_{2}}$ is used to encode the parameter update-rule for training NN achitectures. 
% The full specification of Mnemosyne optimizer is as follows:
At each timestep $t$, gradient $\nabla f(\mathbf{x}_{t})$ is input to the optimizer, for each coordinate independently. The gradient is pre-processed as proposed in \citet{l2l-lstm}  and given to $2$ compact Mnemosyne's memory cells sequentially. The Mnemosyne's memory cell interfaces with the rest of the system similarly to any RNN-cell. Each cell uses exponential discount factor $\tau=0.1$, $r=16$ random projections, $16$ hidden dimensions and $1$ attention head. The memory cell output is fed to a fully connected layer which returns the update to be applied to the NN parameters of the optimizee. 

\textbf{Training details:} 
We refer to training optimizer's parameters $\theta_{2}$ as \textit{meta-training} to distinguish from the optimizee NN training. Mnemosyne's optimizer is meta-trained only on a single ML task: MLP MNIST classifier. The optimizee MLP has $l=1$ hidden layer of size $h=20$ and uses $\mathrm{sigmoid}$ activation function. The optimizee task is to train MLP for $100$ steps on batches of $128$ image-class examples. 
% \vspace{-4mm}
\paragraph{Hybrid loss function to improve generalization:} To promote generalization to new tasks, we use the random-scaling trick proposed by~\citet{kaifeng}. Mnemosyne's optimizer is meta-trained by gradient descent using Adam optimizer with learning rate $\eta=3e-4$ to minimize a combination of two loss functions. The first is the task loss given by the sum of optimizee losses in a truncated roll-out of $5$ MLP training steps. The other one is an imitation loss given by the mean squared error between Mnemosyne's updates and expert-optimizer (Adam) updates for same inputs. Importantly, this imitation loss is different from the one proposed in ~\citet{clearning} which uses off-policy expert roll-outs for imitation. In our case, we provide expert supervision for the on-policy updates. This mitigates the problem of divergence from expert's trajectory, often observed in behaviour cloning. Our imitation loss acts as a regularizer which prevents Mnemosyne's optimizer from over-fitting on the optimizee task that it is trained on.

Our optimizer model has minimal input feature engineering and our meta-training setup is significantly simpler than those considered in the literature~\cite{tasks-stab, clearning, kaifeng, olga}. Even so, we can successfully apply Mnemosyne's optimizer to a variety of tasks due to its efficient memory mechanism. Furthermore, Mnemosyne's memory cells can be easily combined with any of the existing L2L methods that use LSTMs for memory-encoding.

\textbf{Results:}
After meta-training, Mnemosyne's optimizer was tested on NN training tasks with different NN architectures and datasets. Recall that Mnemosyne only saw one ML task of MLP classifier training on MNIST dataset for $100$ steps during meta-training.
Fig. ~\ref{fig:mlp} shows that Mnemosyne can optimize MLPs with different NN archtitectures and activation functions on MNIST image classifier training. Note that, Mnemosyne converges significantly faster than popular analytical optimizers, RMSprop and Adam while retaining similar asymptotic performance. Mnemosyne can train NNs for long horizons of thousands of steps while baseline LSTM optimizer~\cite{l2l-lstm} struggles to minimize classification loss beyond a few hundred steps.

\textbf{Transformers:}  Mnemosyne was also tested on the task of training vision transformers (ViTs) \cite{dosovitskiy} which have significantly different architectures than MLPs. Considered ViT has $3$ attention and MLP layers of size $16$ and $2$ heads. Training curves for image classification with ViTs on different datasets (MNIST, CIFAR10, CIFAR100) are shown in Fig.~\ref{fig:vit}. Here, as before, Mnemosyne's optimizer is faster than standard analytical optimizers and more stable than LSTM optimizer.

\begin{figure}\vspace{-2mm}
\centering
  \includegraphics[width=0.8\linewidth]{img/imitation_comparison_lstm_legend_inside.pdf}
\vspace{-4mm}
\caption{\small{Impact of training the optimizer with combined meta loss and imitation loss can be seen in generalization to a long horizon rollout. All variants were trained only on length $100$ rollouts.}}
\label{fig:imitation}
\vspace{-8mm}
\end{figure}

The stability of Mnemosyne's optimizer is also owed to the on-policy imitation loss for meta-training. Fig.~\ref{fig:imitation} shows the benefit of using expert imitation-loss for long-horizon stability of the Mnemosyne's optimizer.

Our results on training Transformers with Mnemosyne naturally lead to the question of the role that Transformer-based optimizers can play in training Transformers architectures. It is well known that Transformer training requires nontrivial optimization techniques \cite{training-trans}, e.g. learning rate schedulers (for that reason SGD was replaced with Adam in Transformer-training). Furthermore, for larger architectures training is slow, often prohibitively (unless the model is trimmed down, for instance by replacing long-range attention modeling with local attention of the controllable attention radius). Attention-based optimizers can potentially address this problem, since they improve convergence (and thus effectively reduce training time) even if meta-trained on much simpler tasks that do not involve attention-based models, as we show in Fig. \ref{fig:vit}.

\begin{figure*}\vspace{-2mm}
  \includegraphics[width=0.33\textwidth]{img/reg_att_ablation_legend_inside.pdf}
  \includegraphics[width=0.33\textwidth]{img/favorpp_ablation.pdf}
  \includegraphics[width=0.33\textwidth]{img/kernel_ablation.pdf}
\vspace{-8mm}
\caption{\small{Ablation Studies. \textbf{Left:} Comparison of Mnemosyne linear memory with regular attention memory blocks with different history cache lengths ($h$). \textbf{Middle:} Meta-training curves of Mnemosyne optimizer with FAVOR+ and FAVOR++ mechanism. \textbf{Right:} Meta-training curves of Mnemosyne optimizer with different kernel transformation functions.}}
\label{fig:ablations}
\vspace{-2.4mm}
\end{figure*}

\textbf{Ablation studies:}
We have tried to use regular Transformer attention-based decoder blocks to encode memory. For applying regular attention to online optimizer autoregressively, a limited-length cache of historical gradients has to be maintained. A self-attention map over the history sequence is generated and used to encode memory. Fig.~\ref{fig:ablations} (left) shows the meta-training curves for regular attention optimizers with different history cache lengths. As we increase the cache length, the performance improves and the memory requirement scales quadratically. Due to this limitation, we could not implement a regular attention based optimizer with cache length more than $100$. On the other hand, Performer's memory cell can attend to theoretically unbounded history and the finally out-performs regular attention variants with fixed memory requirement.

Fig.~\ref{fig:ablations} (middle) compares the performance of Mnemosyne optimizer with FAVOR+ and FAVOR++ mechanisms explained in Sec.~\ref{sec:algorithms}. FAVOR++ mechanism provides strongest theoretical guarantees for the
capacity of the associative memory model but FAVOR+ performs comparably in practice. Due to the simpler implementation of FAVOR+, we use it for all experiments with Mnemosyne's optimizer.

In Fig.~\ref{fig:ablations}, we compare the performance of Mnemosyne for different maps $\phi$. FAVOR++ mechanism leads initially to faster convergence, but asymptotically performs similarly as the FAVOR+ variant (middle). Optimizers with both regular positive and hyperbolic random features kernel learn similarly, but the latter has much lower variance (right). 
% Both perform better than Relu kernel variant.


